Practice of Streaming Processing of Dynamic Graphs: Concepts, Models, and Systems

Graph processing has become an important part of various areas of computing, including machine learning, medical applications, social network analysis, computational sciences, and others. A growing amount of the associated graph processing workloads are dynamic, with millions of edges added or removed per second. Graph streaming frameworks are specifically crafted to enable the processing of such highly dynamic workloads. Recent years have seen the development of many such frameworks. However, they differ in their general architectures (with key details such as the support for the concurrent execution of graph updates and queries, or the incorporated graph data organization), the types of updates and workloads allowed, and many others. To facilitate the understanding of this growing field, we provide the first analysis and taxonomy of dynamic and streaming graph processing. We focus on identifying the fundamental system designs and on understanding their support for concurrency, and for different graph updates as well as analytics workloads. We also crystallize the meaning of different concepts associated with streaming graph processing, such as dynamic, temporal, online, and time-evolving graphs, edge-centric processing, models for the maintenance of updates, and graph databases. Moreover, we provide a bridge with the very rich landscape of graph streaming theory by giving a broad overview of recent theoretical related advances, and by discussing which graph streaming models and settings could be helpful in developing more powerful streaming frameworks and designs. We also outline graph streaming workloads and research challenges.

==> related.tex <==
\section{Other Works on Dynamic Graphs}

There exist other works on streaming and dynamic graphs that are outside the
core focus of this survey. We outline them as a reference point for the reader.
%
First, different designs target effective \textbf{partitioning of streaming
graph datasets}~\cite{yang2012towards, firth2017loom, firth2016workload,
filippidou2015online, huang2016leopard, shi2017partitioning, hoang2019cusp,
mccrabb2019dredge, pacaci2019experimental}.
%
Second, different works focus on solving a \textbf{specific graph problem in a
streaming setting}. Targeted problems include graph
clustering~\cite{hassani2016hastream}, mining periodic
cliques~\cite{qin2019mining}, search for persistent
communities~\cite{li2018persistent, riedy2013multithreaded}, tracking
conductance~\cite{galhotra2015tracking}, event pattern~\cite{namaki2017event}
and subgraph~\cite{mondal2016casqd} discovery, solving ego-centric
queries~\cite{mondal2014eagr}, pattern
detection~\cite{choudhury2015selectivity, gao2016toward, shao2018efficient,
kim2018turboflux, li2019time, sun2017join, choudhury2018percolator,
gao2014continuous}, densest subgraph identification~\cite{jin2018quickpoint},
frequent subgraph mining~\cite{aslay2018mining},
dense subgraph detection~\cite{ma2017fast}, construction and querying of
knowledge graphs~\cite{choudhury2017nous}, stream
summarization~\cite{gou2019fast}, $k$-core
maintenance~\cite{aksu2014distributed},
shortest paths~\cite{srinivasan2018shared},
Betweenness Centrality~\cite{hayashi2015fully, tripathy2018scaling},
Triangle Counting~\cite{makkar2017exact},
Katz Centrality~\cite{van2018scalable},
Connected Components~\cite{mccoll2013new},
or PageRank~\cite{guo2017parallel}.



\maciej{GraphBolt: Dependency-Driven Synchronous
Processing of Streaming Graphs
%
GraphBolt: Streaming Graph Approximations
https://arxiv.org/pdf/1810.02781.pdf
}

